Horowitz-Manski-Lee Bounds with Multilayered Sample Selection

This paper investigates the causal effect of job training on wage rates in the presence of firm heterogeneity. When training affects the sorting of workers to firms, sample selection is no longer binary but is ``multilayered". This paper extends the canonical Heckman (1979) sample selection model -- which assumes selection is binary -- to a setting where it is multilayered. In this setting Lee bounds set identifies a total effect that combines a weighted-average of the causal effect of job training on wage rates across firms with a weighted-average of the contrast in wages between different firms for a fixed level of training. Thus, Lee bounds set identifies a policy-relevant estimand only when firms pay homogeneous wages and/or when job training does not affect worker sorting across firms. We derive analytic expressions for sharp bounds for the causal effect of job training on wage rates at each firm that leverage information on firm-specific wages. We illustrate our partial identification approach with two empirical applications to job training experiments. Our estimates demonstrate that even when conventional Lee bounds are strictly positive, our within-firm bounds can be tight around 0, showing that the canonical Lee bounds may capture only a pure sorting effect of job training.

==> empiric_tbls_figs/amen_dist/old/scho_t3_wk135_unweighted_A.tex <==
            &        Mean&          S.D.&        Mean&          S.D.&  Difference&          S.E.\\
\midrule
Health insurance&      0.5385&      0.4987&      0.5521&      0.4974&      0.0136&      0.0177\\
Paid sick leave&      0.4599&      0.4986&      0.4561&      0.4982&     -0.0038&      0.0177\\
Paid vacation&      0.6028&      0.4895&      0.5962&      0.4908&     -0.0067&      0.0171\\
Childcare assistance&      0.1300&      0.3364&      0.1411&      0.3482&      0.0111&      0.0121\\
Flexible hours&      0.5570&      0.4969&      0.5793&      0.4938&      0.0223&      0.0174\\
Employer-provided transportation&      0.1969&      0.3978&      0.1813&      0.3854&     -0.0156&      0.0140\\
Pension or retirement benefits&      0.4405&      0.4966&      0.4440&      0.4970&      0.0035&      0.0177\\
Dental plan &      0.4732&      0.4995&      0.4770&      0.4996&      0.0038&      0.0178\\
Tuition reimbursement&      0.2584&      0.4379&      0.2904&      0.4540&      0.0320&      0.0158\\


==> empiric_tbls_figs/amen_dist/old/scho_t3_wk135_unweighted_B.tex <==
 
Employment  &      0.4954&      0.5001&      0.5258&      0.4994&      0.0304&      0.0112\\
Sample size &   3288&           &   5091&           &   8379&           \\


==> empiric_tbls_figs/amen_dist/old/scho_t3_wk180_unweighted_A.tex <==
            &        Mean&          S.D.&        Mean&          S.D.&  Difference&          S.E.\\
\midrule
Health insurance&      0.5547&      0.4972&      0.5737&      0.4946&      0.0191&      0.0155\\
Paid sick leave&      0.4679&      0.4991&      0.4959&      0.5001&      0.0280&      0.0156\\
Paid vacation&      0.6331&      0.4821&      0.6345&      0.4817&      0.0014&      0.0147\\
Childcare assistance&      0.1466&      0.3538&      0.1560&      0.3629&      0.0094&      0.0112\\
Flexible hours&      0.5608&      0.4964&      0.5847&      0.4929&      0.0239&      0.0153\\
Employer-provided transportation&      0.1918&      0.3938&      0.1928&      0.3946&      0.0010&      0.0123\\
Pension or retirement benefits&      0.4453&      0.4972&      0.4749&      0.4995&      0.0296&      0.0156\\
Dental plan &      0.4777&      0.4997&      0.5011&      0.5001&      0.0234&      0.0156\\
Tuition reimbursement&      0.2700&      0.4441&      0.3053&      0.4606&      0.0353&      0.0141\\


==> empiric_tbls_figs/amen_dist/old/scho_t3_wk180_unweighted_B.tex <==
 
Employment  &      0.5307&      0.4991&      0.5655&      0.4957&      0.0348&      0.0111\\
Sample size &   3288&           &   5091&           &   8379&           \\


==> empiric_tbls_figs/amen_dist/old/scho_t3_wk208_unweighted_A.tex <==
            &        Mean&          S.D.&        Mean&          S.D.&  Difference&          S.E.\\
\midrule
Health insurance&      0.5663&      0.4957&      0.5951&      0.4910&      0.0288&      0.0151\\
Paid sick leave&      0.4797&      0.4997&      0.5199&      0.4997&      0.0402&      0.0153\\
Paid vacation&      0.6401&      0.4801&      0.6508&      0.4768&      0.0107&      0.0142\\
Childcare assistance&      0.1500&      0.3572&      0.1656&      0.3717&      0.0156&      0.0111\\
Flexible hours&      0.6039&      0.4892&      0.6097&      0.4879&      0.0058&      0.0147\\
Employer-provided transportation&      0.1959&      0.3970&      0.1975&      0.3982&      0.0016&      0.0121\\
Pension or retirement benefits&      0.4570&      0.4983&      0.4896&      0.5000&      0.0327&      0.0152\\
Dental plan &      0.4936&      0.5001&      0.5209&      0.4997&      0.0273&      0.0153\\
Tuition reimbursement&      0.2953&      0.4563&      0.3160&      0.4650&      0.0206&      0.0140\\


==> empiric_tbls_figs/amen_dist/old/scho_t3_wk208_unweighted_B.tex <==
 
Employment  &      0.5566&      0.4969&      0.5910&      0.4917&      0.0345&      0.0111\\
Sample size &   3288&           &   5091&           &   8379&           \\


==> empiric_tbls_figs/amen_dist/old/scho_t3_wk90_unweighted_A.tex <==
            &        Mean&          S.D.&        Mean&          S.D.&  Difference&          S.E.\\
\midrule
Health insurance&      0.4844&      0.5000&      0.5041&      0.5001&      0.0197&      0.0186\\
Paid sick leave&      0.3916&      0.4883&      0.4224&      0.4941&      0.0308&      0.0183\\
Paid vacation&      0.5369&      0.4988&      0.5761&      0.4943&      0.0392&      0.0181\\
Childcare assistance&      0.1316&      0.3382&      0.1390&      0.3460&      0.0073&      0.0127\\
Flexible hours&      0.5332&      0.4991&      0.5567&      0.4969&      0.0235&      0.0183\\
Employer-provided transportation&      0.2017&      0.4014&      0.1828&      0.3866&     -0.0189&      0.0147\\
Pension or retirement benefits&      0.3696&      0.4829&      0.3916&      0.4882&      0.0219&      0.0180\\
Dental plan &      0.3857&      0.4870&      0.4262&      0.4947&      0.0405&      0.0182\\
Tuition reimbursement&      0.2211&      0.4152&      0.2596&      0.4385&      0.0385&      0.0158\\


==> empiric_tbls_figs/amen_dist/old/scho_t3_wk90_unweighted_B.tex <==
 
Employment  &      0.4386&      0.4963&      0.4410&      0.4966&      0.0024&      0.0111\\
Sample size &   3288&           &   5091&           &   8379&           \\


==> empiric_tbls_figs/amen_dist/old/schochet_t3_wk135.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{cc}}
\toprule
            &     Control&     Treated&  Difference\\
\midrule
Health insurance&       0.539&       0.552&       0.014\\
            &   \{0.499\}&   \{0.497\}&     (0.018)\\
            &            &            &     [0.443]\\
Paid sick leave&       0.460&       0.456&      -0.004\\
            &   \{0.499\}&   \{0.498\}&     (0.018)\\
            &            &            &     [0.831]\\
Paid vacation&       0.603&       0.596&      -0.007\\
            &   \{0.489\}&   \{0.491\}&     (0.017)\\
            &            &            &     [0.697]\\
Childcare assistance&       0.130&       0.141&       0.011\\
            &   \{0.336\}&   \{0.348\}&     (0.012)\\
            &            &            &     [0.364]\\
Flexible hours&       0.557&       0.579&       0.022\\
            &   \{0.497\}&   \{0.494\}&     (0.017)\\
            &            &            &     [0.200]\\
Employer-provided transportation&       0.197&       0.181&      -0.016\\
            &   \{0.398\}&   \{0.385\}&     (0.014)\\
            &            &            &     [0.261]\\
Pension or retirement benefits&       0.440&       0.444&       0.004\\
            &   \{0.497\}&   \{0.497\}&     (0.018)\\
            &            &            &     [0.841]\\
Dental plan &       0.473&       0.477&       0.004\\
            &   \{0.499\}&   \{0.500\}&     (0.018)\\
            &            &            &     [0.829]\\
Tuition reimbursement&       0.258&       0.290&       0.032\\
            &   \{0.438\}&   \{0.454\}&     (0.016)\\
            &            &            &     [0.045]\\
\midrule
Employment  &       0.495&       0.526&       0.030\\
            &     \{0.5\}&   \{0.499\}&     (0.011)\\
            &            &            &     [0.007]\\
Sample Size &        3288&        5091&        8379\\
\bottomrule
\multicolumn{4}{l}{\footnotesize Note: Standard deviations in \{ \}, standard errors in ( ), p-values in [ ].}\\
\end{tabular}
\caption{Probability of working at amenity-providing firm at week 135 (conditional on employment) \label{schoct3135}}
\end{table}


==> empiric_tbls_figs/amen_dist/old/schochet_t3_wk180.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{cc}}
\toprule
            &     Control&     Treated&  Difference\\
\midrule
Health insurance&       0.555&       0.574&       0.019\\
            &   \{0.497\}&   \{0.495\}&     (0.016)\\
            &            &            &     [0.219]\\
Paid sick leave&       0.468&       0.496&       0.028\\
            &   \{0.499\}&   \{0.500\}&     (0.016)\\
            &            &            &     [0.073]\\
Paid vacation&       0.633&       0.635&       0.001\\
            &   \{0.482\}&   \{0.482\}&     (0.015)\\
            &            &            &     [0.926]\\
Childcare assistance&       0.147&       0.156&       0.009\\
            &   \{0.354\}&   \{0.363\}&     (0.011)\\
            &            &            &     [0.405]\\
Flexible hours&       0.561&       0.585&       0.024\\
            &   \{0.496\}&   \{0.493\}&     (0.015)\\
            &            &            &     [0.118]\\
Employer-provided transportation&       0.192&       0.193&       0.001\\
            &   \{0.394\}&   \{0.395\}&     (0.012)\\
            &            &            &     [0.933]\\
Pension or retirement benefits&       0.445&       0.475&       0.030\\
            &   \{0.497\}&   \{0.499\}&     (0.016)\\
            &            &            &     [0.058]\\
Dental plan &       0.478&       0.501&       0.023\\
            &   \{0.500\}&   \{0.500\}&     (0.016)\\
            &            &            &     [0.135]\\
Tuition reimbursement&       0.270&       0.305&       0.035\\
            &   \{0.444\}&   \{0.461\}&     (0.014)\\
            &            &            &     [0.013]\\
\midrule
Employment  &       0.531&       0.566&       0.035\\
            &   \{0.499\}&   \{0.496\}&     (0.011)\\
            &            &            &     [0.002]\\
Sample Size &        3288&        5091&        8379\\
\bottomrule
\multicolumn{4}{l}{\footnotesize Note: Standard deviations in \{ \}, standard errors in ( ), p-values in [ ].}\\
\end{tabular}
\caption{Probability of working at amenity-providing firm at week 180 (conditional on employment) \label{schoct3180}}
\end{table}


==> empiric_tbls_figs/amen_dist/old/schochet_t3_wk208.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{cc}}
\toprule
            &     Control&     Treated&  Difference\\
\midrule
Health insurance&       0.566&       0.595&       0.029\\
            &   \{0.496\}&   \{0.491\}&     (0.015)\\
            &            &            &     [0.056]\\
Paid sick leave&       0.480&       0.520&       0.040\\
            &   \{0.500\}&   \{0.500\}&     (0.015)\\
            &            &            &     [0.008]\\
Paid vacation&       0.640&       0.651&       0.011\\
            &   \{0.480\}&   \{0.477\}&     (0.014)\\
            &            &            &     [0.451]\\
Childcare assistance&       0.150&       0.166&       0.016\\
            &   \{0.357\}&   \{0.372\}&     (0.011)\\
            &            &            &     [0.165]\\
Flexible hours&       0.604&       0.610&       0.006\\
            &   \{0.489\}&   \{0.488\}&     (0.015)\\
            &            &            &     [0.693]\\
Employer-provided transportation&       0.196&       0.198&       0.002\\
            &   \{0.397\}&   \{0.398\}&     (0.012)\\
            &            &            &     [0.895]\\
Pension or retirement benefits&       0.457&       0.490&       0.033\\
            &   \{0.498\}&   \{0.500\}&     (0.015)\\
            &            &            &     [0.032]\\
Dental plan &       0.494&       0.521&       0.027\\
            &   \{0.500\}&   \{0.500\}&     (0.015)\\
            &            &            &     [0.074]\\
Tuition reimbursement&       0.295&       0.316&       0.021\\
            &   \{0.456\}&   \{0.465\}&     (0.014)\\
            &            &            &     [0.143]\\
\midrule
Employment  &       0.557&       0.591&       0.034\\
            &   \{0.497\}&   \{0.492\}&     (0.011)\\
            &            &            &     [0.002]\\
Sample Size &        3288&        5091&        8379\\
\bottomrule
\multicolumn{4}{l}{\footnotesize Note: Standard deviations in \{ \}, standard errors in ( ), p-values in [ ].}\\
\end{tabular}
\caption{Probability of working at amenity-providing firm at week 208 (conditional on employment) \label{schoct3208}}
\end{table}


==> empiric_tbls_figs/amen_dist/old/schochet_t3_wk45.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{cc}}
\toprule
            &     Control&     Treated&  Difference\\
\midrule
Health insurance&       0.405&       0.437&       0.032\\
            &   \{0.491\}&   \{0.496\}&     (0.020)\\
            &            &            &     [0.102]\\
Paid sick leave&       0.337&       0.364&       0.027\\
            &   \{0.473\}&   \{0.481\}&     (0.019)\\
            &            &            &     [0.158]\\
Paid vacation&       0.467&       0.501&       0.034\\
            &   \{0.499\}&   \{0.500\}&     (0.019)\\
            &            &            &     [0.075]\\
Childcare assistance&       0.102&       0.118&       0.016\\
            &   \{0.303\}&   \{0.322\}&     (0.013)\\
            &            &            &     [0.209]\\
Flexible hours&       0.576&       0.597&       0.021\\
            &   \{0.494\}&   \{0.491\}&     (0.019)\\
            &            &            &     [0.266]\\
Employer-provided transportation&       0.213&       0.197&      -0.016\\
            &   \{0.410\}&   \{0.398\}&     (0.016)\\
            &            &            &     [0.305]\\
Pension or retirement benefits&       0.298&       0.328&       0.030\\
            &   \{0.458\}&   \{0.470\}&     (0.019)\\
            &            &            &     [0.114]\\
Dental plan &       0.301&       0.332&       0.032\\
            &   \{0.459\}&   \{0.471\}&     (0.018)\\
            &            &            &     [0.088]\\
Tuition reimbursement&       0.195&       0.228&       0.033\\
            &   \{0.397\}&   \{0.420\}&     (0.016)\\
            &            &            &     [0.043]\\
\midrule
Employment  &       0.403&       0.322&      -0.080\\
            &   \{0.491\}&   \{0.467\}&     (0.011)\\
            &            &            &     [0.000]\\
Sample Size &        3288&        5091&        8379\\
\bottomrule
\multicolumn{4}{l}{\footnotesize Note: Standard deviations in \{ \}, standard errors in ( ), p-values in [ ]}\\
\end{tabular}
\caption{Probability of working at amenity-providing firm at week 45 (conditional on employment) \label{schoct345}}
\end{table}


==> empiric_tbls_figs/amen_dist/old/schochet_t3_wk90.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{cc}}
\toprule
            &     Control&     Treated&  Difference\\
\midrule
Health insurance&       0.484&       0.504&       0.020\\
            &   \{0.500\}&   \{0.500\}&     (0.019)\\
            &            &            &     [0.291]\\
Paid sick leave&       0.392&       0.422&       0.031\\
            &   \{0.488\}&   \{0.494\}&     (0.018)\\
            &            &            &     [0.092]\\
Paid vacation&       0.537&       0.576&       0.039\\
            &   \{0.499\}&   \{0.494\}&     (0.018)\\
            &            &            &     [0.030]\\
Childcare assistance&       0.132&       0.139&       0.007\\
            &   \{0.338\}&   \{0.346\}&     (0.013)\\
            &            &            &     [0.565]\\
Flexible hours&       0.533&       0.557&       0.024\\
            &   \{0.499\}&   \{0.497\}&     (0.018)\\
            &            &            &     [0.199]\\
Employer-provided transportation&       0.202&       0.183&      -0.019\\
            &   \{0.401\}&   \{0.387\}&     (0.015)\\
            &            &            &     [0.196]\\
Pension or retirement benefits&       0.370&       0.392&       0.022\\
            &   \{0.483\}&   \{0.488\}&     (0.018)\\
            &            &            &     [0.225]\\
Dental plan &       0.386&       0.426&       0.041\\
            &   \{0.487\}&   \{0.495\}&     (0.018)\\
            &            &            &     [0.027]\\
Tuition reimbursement&       0.221&       0.260&       0.039\\
            &   \{0.415\}&   \{0.439\}&     (0.016)\\
            &            &            &     [0.016]\\
\midrule
Employment  &       0.439&       0.441&       0.002\\
            &   \{0.496\}&   \{0.497\}&     (0.011)\\
            &            &            &   [0.00828]\\
Sample Size &        3288&        5091&        8379\\
\bottomrule
\multicolumn{4}{l}{\footnotesize Note: Standard deviations in \{ \}, standard errors in ( ), p-values in [ ].}\\
\end{tabular}
\caption{Probability of working at amenity-providing firm at week 90 (conditional on employment) \label{schoct390}}
\end{table}


==> empiric_tbls_figs/bounds/old/health_wk135_bounds.tex <==
\\
\midrule
Baseline &      0.0355&      0.0000&     -1.1192&      1.1244&           &           \\
 $p_{H,H} \geq p_{H,L} $           &      0.1387&      0.0767&     -0.5117&      0.5353&     -0.6159&      0.7046\\
(H,L) is smallest type&      0.2641&      0.2154&     -0.1161&      0.1280&     -0.1224&      0.1598\\
$p_{H,L} = 0$&      0.2774&      0.2154&     -0.0578&      0.0673&     -0.1224&      0.1598\\


==> empiric_tbls_figs/bounds/old/health_wk135_phh_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.035&       \scriptsize $ P(D=H|Z=0)-P(D=L|Z=1) $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.139&       \scriptsize $ P(D=H|Z=0)/2 $\\
Asm. (H,L) is smallest type&       0.264&       \tiny $ (3 P(D=H|Z=0) + P(D=L|Z=0) - P(D=H|Z=1) - P(D=L|Z=1))/2 $\\
Asm. P(T=(H,L)) = 0&       0.277&       \scriptsize $ P(D=H|Z=0) $\\


==> empiric_tbls_figs/bounds/old/health_wk135_pll_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.000&       \scriptsize $ 0 $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.077&       \scriptsize $ P(D=H|Z=0)/2 - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. (H,L) is smallest type&       0.215&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. P(T=(H,L)) = 0&       0.215&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\


==> empiric_tbls_figs/bounds/old/health_wk180_bounds.tex <==
\\
\midrule
Baseline &      0.0472&      0.0000&     -1.0134&      1.0841&           &           \\
 $p_{H,H} \geq p_{H,L} $           &      0.1499&      0.0677&     -0.5049&      0.5399&     -0.7433&      0.8143\\
(H,L) is smallest type&      0.2823&      0.2176&     -0.1258&      0.1438&     -0.1618&      0.1846\\
$p_{H,L} = 0$&      0.2997&      0.2176&     -0.0506&      0.0724&     -0.1618&      0.1846\\


==> empiric_tbls_figs/bounds/old/health_wk180_phh_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.047&       \scriptsize $ P(D=H|Z=0)-P(D=L|Z=1) $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.150&       \scriptsize $ P(D=H|Z=0)/2 $\\
Asm. (H,L) is smallest type&       0.282&       \tiny $ (3 P(D=H|Z=0) + P(D=L|Z=0) - P(D=H|Z=1) - P(D=L|Z=1))/2 $\\
Asm. P(T=(H,L)) = 0&       0.300&       \scriptsize $ P(D=H|Z=0) $\\


==> empiric_tbls_figs/bounds/old/health_wk180_pll_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.000&       \scriptsize $ 0 $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.068&       \scriptsize $ P(D=H|Z=0)/2 - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. (H,L) is smallest type&       0.218&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. P(T=(H,L)) = 0&       0.218&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\


==> empiric_tbls_figs/bounds/old/health_wk208_bounds.tex <==
\\
\midrule
Baseline &      0.0683&      0.0000&     -0.8568&      0.9515&           &           \\
 $p_{H,H} \geq p_{H,L} $           &      0.1596&      0.0547&     -0.4884&      0.5580&     -0.8894&      0.8629\\
(H,L) is smallest type&      0.3008&      0.2143&     -0.1128&      0.1622&     -0.1826&      0.1911\\
$p_{H,L} = 0$&      0.3191&      0.2143&     -0.0409&      0.0931&     -0.1826&      0.1911\\


==> empiric_tbls_figs/bounds/old/health_wk208_phh_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.068&       \scriptsize $ P(D=H|Z=0)-P(D=L|Z=1) $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.160&       \scriptsize $ P(D=H|Z=0)/2 $\\
Asm. (H,L) is smallest type&       0.301&       \tiny $ (3 P(D=H|Z=0) + P(D=L|Z=0) - P(D=H|Z=1) - P(D=L|Z=1))/2 $\\
Asm. P(T=(H,L)) = 0&       0.319&       \scriptsize $ P(D=H|Z=0) $\\


==> empiric_tbls_figs/bounds/old/health_wk208_pll_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.000&       \scriptsize $ 0 $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.055&       \scriptsize $ P(D=H|Z=0)/2 - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. (H,L) is smallest type&       0.214&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. P(T=(H,L)) = 0&       0.214&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\


==> empiric_tbls_figs/bounds/old/health_wk45_bounds.tex <==
\\
\midrule
Baseline &      0.0000&      0.1004&           &           &     -0.4163&      0.4630\\
 $p_{H,H} \geq p_{H,L} $          &      0.0865&      0.1870&     -0.3599&      0.4249&     -0.1191&      0.1780\\
(H,L) is smallest type&      0.2126&      0.2735&           &           &           &           \\
$p_{H,L} = 0$ &      0.1731&      0.2735&           &           &           &           \\


==> empiric_tbls_figs/bounds/old/health_wk45_phh_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.000&       \scriptsize $ 0 $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.087&       \scriptsize $ P(D=H|Z=0)/2 $\\
Asm. (H,L) is smallest type&       0.213&       \tiny $ (3 P(D=H|Z=0) + P(D=L|Z=0) - P(D=H|Z=1) - P(D=L|Z=1))/2 $\\
Asm. P(T=(H,L)) = 0&       0.173&       \scriptsize $ P(D=H|Z=0) $\\


==> empiric_tbls_figs/bounds/old/health_wk45_pll_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.100&       \scriptsize $ P(D=L|Z=0) - P(D=H|Z=1) $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.187&       \scriptsize $ P(D=H|Z=0)/2 - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. (H,L) is smallest type&       0.274&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. P(T=(H,L)) = 0&       0.274&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\


==> empiric_tbls_figs/bounds/old/health_wk90_bounds.tex <==
\\
\midrule
Baseline &      0.0000&      0.0018&           &           &     -2.5438&      2.5354\\
 $p_{H,H} \geq p_{H,L} $           &      0.1112&      0.1130&     -0.4327&      0.4961&     -0.3990&      0.4473\\
(H,L) is smallest type&      0.2219&      0.2243&     -0.0180&      0.0720&     -0.0296&      0.0738\\
$p_{H,L} = 0$&      0.2225&      0.2243&     -0.0139&      0.0684&     -0.0296&      0.0738\\


==> empiric_tbls_figs/bounds/old/health_wk90_phh_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.000&       \scriptsize $ 0 $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.111&       \scriptsize $ P(D=H|Z=0)/2 $\\
Asm. (H,L) is smallest type&       0.222&       \tiny $ (3 P(D=H|Z=0) + P(D=L|Z=0) - P(D=H|Z=1) - P(D=L|Z=1))/2 $\\
Asm. P(T=(H,L)) = 0&       0.222&       \scriptsize $ P(D=H|Z=0) $\\


==> empiric_tbls_figs/bounds/old/health_wk90_pll_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.002&       \scriptsize $ P(D=L|Z=0) - P(D=H|Z=1) $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.113&       \scriptsize $ P(D=H|Z=0)/2 - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. (H,L) is smallest type&       0.224&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. P(T=(H,L)) = 0&       0.224&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\


==> empiric_tbls_figs/bounds/old/lee_bounds.tex <==
            &  $\mathbb P[D>0|Z=0]$ &  $\mathbb P[D>0|Z=1]$ &$p$&      lower&       upper\\
\midrule
%Week 45     &      0.4240&      0.3449&      0.1865&     -0.0849&      0.1230\\
Week 90     &      0.4612&      0.4623&      0.0023&      0.0315&      0.0409\\
Week 135    &      0.5204&      0.5469&      0.0484&     -0.0156&      0.0728\\
Week 180    &      0.5482&      0.5831&      0.0599&     -0.0305&      0.0780\\
Week 208    &      0.5713&      0.6078&      0.0601&     -0.0230&      0.0878\\


==> empiric_tbls_figs/bounds/old/pension_wk135_bounds.tex <==
\\
\midrule
Baseline &      0.0000&      0.0405&           &           &     -1.0007&      1.0887\\
 $p_{H,H} \geq p_{H,L} $          &      0.1158&      0.1563&     -0.4770&      0.5642&     -0.4453&      0.4460\\
(H,L) is smallest type&      0.2183&      0.2721&     -0.0812&      0.1571&     -0.1208&      0.1023\\
$p_{H,L} = 0$ &      0.2315&      0.2721&     -0.0120&      0.0854&     -0.1208&      0.1023\\


==> empiric_tbls_figs/bounds/old/pension_wk135_phh_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.000&       \scriptsize $ 0 $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.116&       \scriptsize $ P(D=H|Z=0)/2 $\\
Asm. (H,L) is smallest type&       0.218&       \tiny $ (3 P(D=H|Z=0) + P(D=L|Z=0) - P(D=H|Z=1) - P(D=L|Z=1))/2 $\\
Asm. P(T=(H,L)) = 0&       0.232&       \scriptsize $ P(D=H|Z=0) $\\


==> empiric_tbls_figs/bounds/old/pension_wk135_pll_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.041&       \scriptsize $ P(D=L|Z=0) - P(D=H|Z=1) $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.156&       \scriptsize $ P(D=H|Z=0)/2 - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. (H,L) is smallest type&       0.272&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. P(T=(H,L)) = 0&       0.272&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\


==> empiric_tbls_figs/bounds/old/pension_wk180_bounds.tex <==
\\
\midrule
Baseline &      0.0000&      0.0373&           &           &     -1.1495&      1.2423\\
 $p_{H,H} \geq p_{H,L} $          &      0.1185&      0.1558&     -0.5203&      0.5543&     -0.4828&      0.5092\\
(H,L) is smallest type&      0.2195&      0.2743&     -0.1578&      0.1795&     -0.1500&      0.1689\\
$p_{H,L} = 0$&      0.2370&      0.2743&     -0.0760&      0.0919&     -0.1500&      0.1689\\


==> empiric_tbls_figs/bounds/old/pension_wk180_phh_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.000&       \scriptsize $ 0 $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.118&       \scriptsize $ P(D=H|Z=0)/2 $\\
Asm. (H,L) is smallest type&       0.219&       \tiny $ (3 P(D=H|Z=0) + P(D=L|Z=0) - P(D=H|Z=1) - P(D=L|Z=1))/2 $\\
Asm. P(T=(H,L)) = 0&       0.237&       \scriptsize $ P(D=H|Z=0) $\\


==> empiric_tbls_figs/bounds/old/pension_wk180_pll_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.037&       \scriptsize $ P(D=L|Z=0) - P(D=H|Z=1) $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.156&       \scriptsize $ P(D=H|Z=0)/2 - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. (H,L) is smallest type&       0.274&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. P(T=(H,L)) = 0&       0.274&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\


==> empiric_tbls_figs/bounds/old/pension_wk208_bounds.tex <==
\\
\midrule
Baseline &      0.0000&      0.0270&           &           &     -1.4190&      1.4419\\
 $p_{H,H} \geq p_{H,L} $           &      0.1255&      0.1524&     -0.4972&      0.5421&     -0.5108&      0.5292\\
(H,L) is smallest type&      0.2326&      0.2779&     -0.1470&      0.1842&     -0.1586&      0.1788\\
$p_{H,L} = 0$ &      0.2509&      0.2779&     -0.0717&      0.1001&     -0.1586&      0.1788\\


==> empiric_tbls_figs/bounds/old/pension_wk208_phh_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.000&       \scriptsize $ 0 $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.125&       \scriptsize $ P(D=H|Z=0)/2 $\\
Asm. (H,L) is smallest type&       0.233&       \tiny $ (3 P(D=H|Z=0) + P(D=L|Z=0) - P(D=H|Z=1) - P(D=L|Z=1))/2 $\\
Asm. P(T=(H,L)) = 0&       0.251&       \scriptsize $ P(D=H|Z=0) $\\


==> empiric_tbls_figs/bounds/old/pension_wk208_pll_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.027&       \scriptsize $ P(D=L|Z=0) - P(D=H|Z=1) $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.152&       \scriptsize $ P(D=H|Z=0)/2 - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. (H,L) is smallest type&       0.278&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. P(T=(H,L)) = 0&       0.278&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\


==> empiric_tbls_figs/bounds/old/pension_wk45_bounds.tex <==
\\
\midrule
Baseline &      0.0000&      0.1812&           &           &     -0.2266&      0.3013\\
 $p_{H,H} \geq p_{H,L} $        &      0.0644&      0.2455&     -0.4141&      0.4487&           &           \\
(H,L) is smallest type&      0.1683&      0.3099&           &           &           &           \\
$p_{H,L}=0$ &      0.1288&      0.3099&           &           &           &           \\


==> empiric_tbls_figs/bounds/old/pension_wk45_phh_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.000&       \scriptsize $ 0 $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.064&       \scriptsize $ P(D=H|Z=0)/2 $\\
Asm. (H,L) is smallest type&       0.168&       \tiny $ (3 P(D=H|Z=0) + P(D=L|Z=0) - P(D=H|Z=1) - P(D=L|Z=1))/2 $\\
Asm. P(T=(H,L)) = 0&       0.129&       \scriptsize $ P(D=H|Z=0) $\\


==> empiric_tbls_figs/bounds/old/pension_wk45_pll_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.181&       \scriptsize $ P(D=L|Z=0) - P(D=H|Z=1) $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.246&       \scriptsize $ P(D=H|Z=0)/2 - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. (H,L) is smallest type&       0.310&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. P(T=(H,L)) = 0&       0.310&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\


==> empiric_tbls_figs/bounds/old/pension_wk90_bounds.tex <==
\\
\midrule
Baseline &      0.0000&      0.1062&           &           &     -0.5036&      0.5540\\
 $p_{H,H} \geq p_{H,L} $           &      0.0851&      0.1913&     -0.4589&      0.5272&     -0.2588&      0.3021\\
(H,L) is smallest type&      0.1697&      0.2764&     -0.0284&      0.0855&     -0.0233&      0.0655\\
$p_{H,L} = 0$&      0.1703&      0.2764&     -0.0231&      0.0813&     -0.0233&      0.0655\\


==> empiric_tbls_figs/bounds/old/pension_wk90_phh_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.000&       \scriptsize $ 0 $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.085&       \scriptsize $ P(D=H|Z=0)/2 $\\
Asm. (H,L) is smallest type&       0.170&       \tiny $ (3 P(D=H|Z=0) + P(D=L|Z=0) - P(D=H|Z=1) - P(D=L|Z=1))/2 $\\
Asm. P(T=(H,L)) = 0&       0.170&       \scriptsize $ P(D=H|Z=0) $\\


==> empiric_tbls_figs/bounds/old/pension_wk90_pll_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.106&       \scriptsize $ P(D=L|Z=0) - P(D=H|Z=1) $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.191&       \scriptsize $ P(D=H|Z=0)/2 - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. (H,L) is smallest type&       0.276&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. P(T=(H,L)) = 0&       0.276&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\


==> empiric_tbls_figs/bounds/old/vacat_wk135_bounds.tex <==
\\
\midrule
Baseline &      0.0849&      0.0000&     -0.8055&      0.8673&           &           \\
 $p_{H,H} \geq p_{H,L} $          &      0.1548&      0.0435&     -0.5167&      0.5704&     -0.8693&      0.9528\\
(H,L) is smallest type&      0.2972&      0.1983&     -0.0807&      0.1227&     -0.1317&      0.1325\\
$p_{H,L}= 0$ &      0.3097&      0.1983&     -0.0119&      0.0660&     -0.1317&      0.1325\\


==> empiric_tbls_figs/bounds/old/vacat_wk135_phh_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.085&       \scriptsize $ P(D=H|Z=0)-P(D=L|Z=1) $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.155&       \scriptsize $ P(D=H|Z=0)/2 $\\
Asm. (H,L) is smallest type&       0.297&       \scriptsize $ 2 P(D=H|Z=0) - P(D=H|Z=1) $\\
Asm. P(T=(H,L)) = 0&       0.310&       \scriptsize $ P(D=H|Z=0) $\\


==> empiric_tbls_figs/bounds/old/vacat_wk135_pll_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.000&       \scriptsize $ 0 $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.043&       \scriptsize $ P(D=H|Z=0)/2 - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. (H,L) is smallest type&       0.198&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. P(T=(H,L)) = 0&       0.198&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\


==> empiric_tbls_figs/bounds/old/vacat_wk180_bounds.tex <==
\\
\midrule
Baseline &      0.1153&      0.0000&     -0.7220&      0.7650&           &           \\
 $p_{H,H} \geq p_{H,L} $           &      0.1698&      0.0196&     -0.5241&      0.5694&     -1.4437&      1.5135\\
(H,L) is smallest type&      0.3221&      0.1893&     -0.1063&      0.1381&     -0.1713&      0.1852\\
$p_{H,L}= 0$ &      0.3395&      0.1893&     -0.0282&      0.0683&     -0.1713&      0.1852\\


==> empiric_tbls_figs/bounds/old/vacat_wk180_phh_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.115&       \scriptsize $ P(D=H|Z=0)-P(D=L|Z=1) $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.170&       \scriptsize $ P(D=H|Z=0)/2 $\\
Asm. (H,L) is smallest type&       0.322&       \tiny $ (3 P(D=H|Z=0) + P(D=L|Z=0) - P(D=H|Z=1) - P(D=L|Z=1))/2 $\\
Asm. P(T=(H,L)) = 0&       0.340&       \scriptsize $ P(D=H|Z=0) $\\


==> empiric_tbls_figs/bounds/old/vacat_wk180_pll_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.000&       \scriptsize $ 0 $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.020&       \scriptsize $ P(D=H|Z=0)/2 - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. (H,L) is smallest type&       0.189&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. P(T=(H,L)) = 0&       0.189&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\


==> empiric_tbls_figs/bounds/old/vacat_wk208_bounds.tex <==
\\
\midrule
Baseline &      0.1338&      0.0000&     -0.6584&      0.7363&           &           \\
 $p_{H,H} \geq p_{H,L} $           &      0.1781&      0.0077&     -0.5132&      0.5916&     -2.4513&      2.3350\\
(H,L) is smallest type&      0.3378&      0.1857&     -0.1044&      0.1646&     -0.1988&      0.2069\\
$p_{H,L}=0$ &      0.3561&      0.1857&     -0.0229&      0.0969&     -0.1988&      0.2069\\


==> empiric_tbls_figs/bounds/old/vacat_wk208_phh_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.134&       \scriptsize $ P(D=H|Z=0)-P(D=L|Z=1) $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.178&       \scriptsize $ P(D=H|Z=0)/2 $\\
Asm. (H,L) is smallest type&       0.338&       \tiny $ (3 P(D=H|Z=0) + P(D=L|Z=0) - P(D=H|Z=1) - P(D=L|Z=1))/2 $\\
Asm. P(T=(H,L)) = 0&       0.356&       \scriptsize $ P(D=H|Z=0) $\\


==> empiric_tbls_figs/bounds/old/vacat_wk208_pll_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.000&       \scriptsize $ 0 $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.008&       \scriptsize $ P(D=H|Z=0)/2 - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. (H,L) is smallest type&       0.186&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. P(T=(H,L)) = 0&       0.186&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\


==> empiric_tbls_figs/bounds/old/vacat_wk45_bounds.tex <==
\\
\midrule
Baseline &      0.0220&      0.0571&     -1.2826&      1.2191&     -0.6410&      0.7351\\
 $p_{H,H} \geq p_{H,L} $           &      0.0978&      0.1549&     -0.4612&      0.4745&     -0.1885&      0.2512\\
(H,L) is smallest type&      0.2351&      0.2527&           &           &           &           \\
$p{H,L} = 0$ &      0.1956&      0.2527&           &           &           &           \\


==> empiric_tbls_figs/bounds/old/vacat_wk45_phh_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.022&       \scriptsize $ P(D=H|Z=0)-P(D=L|Z=1) $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.098&       \scriptsize $ P(D=H|Z=0)/2 $\\
Asm. (H,L) is smallest type&       0.235&       \tiny $ (3 P(D=H|Z=0) + P(D=L|Z=0) - P(D=H|Z=1) - P(D=L|Z=1))/2 $\\
Asm. P(T=(H,L)) = 0&       0.196&       \scriptsize $ P(D=H|Z=0) $\\


==> empiric_tbls_figs/bounds/old/vacat_wk45_pll_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.057&       \scriptsize $ P(D=L|Z=0) - P(D=H|Z=1) $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.155&       \scriptsize $ P(D=H|Z=0)/2 - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. (H,L) is smallest type&       0.253&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. P(T=(H,L)) = 0&       0.253&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\


==> empiric_tbls_figs/bounds/old/vacat_wk90_bounds.tex <==
\\
\midrule
Baseline &      0.0488&      0.0000&     -0.9443&      1.0260&           &           \\
 $p_{H,H} \geq p_{H,L} $          &      0.1223&      0.0724&     -0.5183&      0.5585&     -0.5422&      0.6165\\
(H,L) is smallest type&      0.2440&      0.1947&     -0.0481&      0.0941&     -0.0390&      0.1074\\
$p_{H,L} = 0$ &      0.2445&      0.1947&     -0.0400&      0.0886&     -0.0390&      0.1074\\


==> empiric_tbls_figs/bounds/old/vacat_wk90_phh_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.049&       \scriptsize $ P(D=H|Z=0)-P(D=L|Z=1) $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.122&       \scriptsize $ P(D=H|Z=0)/2 $\\
Asm. (H,L) is smallest type&       0.244&       \tiny $ (3 P(D=H|Z=0) + P(D=L|Z=0) - P(D=H|Z=1) - P(D=L|Z=1))/2 $\\
Asm. P(T=(H,L)) = 0&       0.245&       \scriptsize $ P(D=H|Z=0) $\\


==> empiric_tbls_figs/bounds/old/vacat_wk90_pll_argmaxes.tex <==
\\
\midrule
No additional assumptions&       0.000&       \scriptsize $ 0 $\\
Asm. P(T=(H,H)) $ \geq $ P(T=(H,L))         &       0.072&       \scriptsize $ P(D=H|Z=0)/2 - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. (H,L) is smallest type&       0.195&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\
Asm. P(T=(H,L)) = 0&       0.195&       \scriptsize $ P(D=H|Z=0) - P(D=H|Z=1) + P(D=L|Z=0) $\\


==> empiric_tbls_figs/pscores/old/health_pscores.tex <==
            &  $\mathbb P[D=H|Z=0]$ & $\mathbb P[D=H|Z=1]$&  $\mathbb P[D=L|Z=0]$&  $\mathbb P[D=L|Z=1]$\\
\midrule
%Week 45     &      0.1731&      0.1505&      0.2509&      0.1945\\
Week 90     &      0.2225&      0.2370&      0.2388&      0.2254\\
Week 135    &      0.2774&      0.3050&      0.2431&      0.2419\\
Week 180    &      0.2997&      0.3306&      0.2485&      0.2525\\
Week 208    &      0.3191&      0.3570&      0.2522&      0.2509\\


==> empiric_tbls_figs/pscores/old/pension_pscores.tex <==
   &  $\mathbb P[D=H|Z=0]$ & $\mathbb P[D=H|Z=1]$&  $\mathbb P[D=L|Z=0]$&  $\mathbb P[D=L|Z=1]$\\
\midrule
%Week 45     &      0.1288&      0.1141&      0.2952&      0.2309\\
Week 90     &      0.1703&      0.1848&      0.2910&      0.2775\\
Week 135    &      0.2315&      0.2483&      0.2889&      0.2985\\
Week 180    &      0.2370&      0.2739&      0.3113&      0.3092\\
Week 208    &      0.2509&      0.2934&      0.3204&      0.3144\\


==> empiric_tbls_figs/pscores/old/vacat_pscores.tex <==
   &  $\mathbb P[D=H|Z=0]$ & $\mathbb P[D=H|Z=1]$&  $\mathbb P[D=L|Z=0]$&  $\mathbb P[D=L|Z=1]$\\
\midrule
%Week 45     &      0.1956&      0.1713&      0.2284&      0.1736\\
Week 90     &      0.2445&      0.2666&      0.2167&      0.1957\\
Week 135    &      0.3097&      0.3221&      0.2108&      0.2248\\
Week 180    &      0.3395&      0.3589&      0.2087&      0.2243\\
Week 208    &      0.3561&      0.3855&      0.2151&      0.2223\\


==> empiric_tbls_figs/sum_stats/old/lee_table1_sumstats.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{7}{ccccc}}
\toprule
                    &     Control&        S.D.&     Treated&        S.D.&  Difference&        S.E.&     P-value\\
\midrule
White, non-Hispanic &        0.26&        0.44&        0.26&        0.44&        0.00&        0.01&        0.96\\
Black, non-Hispanic &        0.50&        0.50&        0.50&        0.50&        0.00&        0.01&        0.90\\
Hispanic            &        0.17&        0.38&        0.17&        0.38&       -0.00&        0.01&        0.89\\
Other race/ethnicity&        0.07&        0.26&        0.07&        0.26&       -0.00&        0.01&        0.89\\
Never married       &        0.92&        0.27&        0.91&        0.28&       -0.01&        0.01&        0.26\\
Married             &        0.02&        0.15&        0.02&        0.15&       -0.00&        0.00&        1.00\\
Living together     &        0.04&        0.20&        0.04&        0.20&        0.00&        0.00&        0.62\\
Separated           &        0.02&        0.14&        0.03&        0.16&        0.00&        0.00&        0.15\\
Education           &       10.09&        1.53&       10.14&        1.57&        0.04&        0.03&        0.22\\
Mother's education  &       11.49&        2.59&       11.47&        2.58&       -0.01&        0.06&        0.82\\
Ever arrested       &        0.26&        0.44&        0.24&        0.43&       -0.01&        0.01&        0.12\\
\textbf{Household income} & & & & & & & \\
$ < $3,000          &        0.25&        0.43&        0.26&        0.44&        0.01&        0.01&        0.39\\
3,000-6,000         &        0.21&        0.41&        0.21&        0.41&        0.00&        0.01&        0.88\\
6,000-9,000         &        0.11&        0.32&        0.12&        0.32&        0.00&        0.01&        0.67\\
9,000-18,000        &        0.25&        0.43&        0.24&        0.43&       -0.00&        0.01&        0.70\\
$ > $18,000         &        0.18&        0.39&        0.17&        0.38&       -0.01&        0.01&        0.29\\
\textbf{Personal income} & & & & & & & \\
$ < $3,000          &        0.79&        0.41&        0.78&        0.41&       -0.00&        0.01&        0.64\\
3,000-6,000         &        0.13&        0.34&        0.13&        0.34&        0.00&        0.01&        0.93\\
6,000-9,000         &        0.05&        0.21&        0.05&        0.23&        0.01&        0.00&        0.15\\
$ > $9,000          &        0.04&        0.18&        0.03&        0.18&       -0.00&        0.00&        0.39\\
\textbf{At baseline} & & & & & & & \\
Have job            &        0.19&        0.39&        0.20&        0.40&        0.01&        0.01&        0.53\\
Mths. empl. prev. yr.&        3.52&        4.23&        3.59&        4.26&        0.06&        0.09&        0.49\\
Had job, prev. yr.  &        0.63&        0.48&        0.63&        0.48&        0.00&        0.01&        0.71\\
Earnings, prev. yr. &     2834.08&     4496.93&     2889.50&     6306.44&       55.43&      125.37&        0.66\\
Usual hours/week    &       21.02&       20.79&       21.67&       21.01&        0.65&        0.45&        0.15\\
Usual weekly earn.  &      104.03&      117.69&      109.92&      343.24&        5.90&        5.94&        0.32\\
\textbf{Post randomization} & & & & & & & \\
Week 52 hours       &       17.95&       23.65&       15.27&       22.56&       -2.68&        0.49&        0.00\\
Week 104 hours      &       22.25&       26.29&       22.57&       26.14&        0.32&        0.56&        0.57\\
Week 156 hours      &       24.20&       26.37&       25.84&       26.45&        1.64&        0.57&        0.00\\
Week 208 hours      &       26.39&       26.58&       27.71&       25.61&        1.32&        0.56&        0.02\\
Week 52 earn.       &      105.96&      164.23&       91.55&      149.13&      -14.41&        3.32&        0.00\\
Week 104 earn.      &      153.03&      208.69&      156.76&      199.05&        3.73&        4.34&        0.39\\
Week 156 earn.      &      184.63&      228.29&      203.69&      239.45&       19.06&        5.03&        0.00\\
Week 208 earn.      &      206.53&      235.41&      227.52&      249.33&       20.99&        5.22&        0.00\\
Total 4 yr. earn.   &    30659.18&    27365.85&    30773.50&    26403.90&      114.32&      573.36&        0.84\\
\midrule
Sample Size         &        3599&            &        5546&            &        9145&            &            \\
\bottomrule
\multicolumn{8}{l}{\footnotesize Note: Weekly earnings calculated as the sum of total earnings in a given week; weekly earnings are not}\\
\multicolumn{8}{l}{\footnotesize conditional on employment and therefore include 0s for the unemployed.} \\
\end{tabular}
\caption{Summary statistics by treatment status \label{sumstats}}
\end{table}


==> empiric_tbls_figs/sum_stats/old/sumstats_unweighted_1.tex <==
            &        Mean&          S.D.&        Mean&          S.D.&  Difference&          S.E.\\
\midrule
White, non-Hispanic&        0.26&        0.44&        0.26&        0.44&        0.00&        0.01\\
Black, non-Hispanic&        0.50&        0.50&        0.50&        0.50&        0.00&        0.01\\
Hispanic    &        0.17&        0.38&        0.17&        0.38&       -0.00&        0.01\\
Other race/ethnicity&        0.07&        0.26&        0.07&        0.26&       -0.00&        0.01\\
Never married&        0.92&        0.27&        0.91&        0.28&       -0.01&        0.01\\
Married     &        0.02&        0.15&        0.02&        0.15&       -0.00&        0.00\\
Living together&        0.04&        0.20&        0.04&        0.20&        0.00&        0.00\\
Separated   &        0.02&        0.14&        0.03&        0.16&        0.00&        0.00\\
Education   &       10.09&        1.53&       10.14&        1.57&        0.04&        0.03\\
Mother's education&       11.49&        2.59&       11.47&        2.58&       -0.01&        0.06\\
Ever arrested&        0.26&        0.44&        0.24&        0.43&       -0.01&        0.01\\


==> empiric_tbls_figs/sum_stats/old/sumstats_unweighted_2.tex <==
 
$ < $3,000  &        0.25&        0.43&        0.26&        0.44&        0.01&        0.01\\
3,000-6,000 &        0.21&        0.41&        0.21&        0.41&        0.00&        0.01\\
6,000-9,000 &        0.11&        0.32&        0.12&        0.32&        0.00&        0.01\\
9,000-18,000&        0.25&        0.43&        0.24&        0.43&       -0.00&        0.01\\
$ > $18,000 &        0.18&        0.39&        0.17&        0.38&       -0.01&        0.01\\


==> empiric_tbls_figs/sum_stats/old/sumstats_unweighted_3.tex <==
 
$ < $3,000  &        0.79&        0.41&        0.78&        0.41&       -0.00&        0.01\\
3,000-6,000 &        0.13&        0.34&        0.13&        0.34&        0.00&        0.01\\
6,000-9,000 &        0.05&        0.21&        0.05&        0.23&        0.01&        0.00\\
$ > $9,000  &        0.04&        0.18&        0.03&        0.18&       -0.00&        0.00\\


==> empiric_tbls_figs/sum_stats/old/sumstats_unweighted_4.tex <==
 
Have job    &        0.19&        0.39&        0.20&        0.40&        0.01&        0.01\\
Mths. empl. prev. yr.&        3.52&        4.23&        3.59&        4.26&        0.06&        0.09\\
Had job, prev. yr.&        0.63&        0.48&        0.63&        0.48&        0.00&        0.01\\
Earnings, prev. yr.&     2834.08&     4496.93&     2889.50&     6306.44&       55.43&      116.81\\
Usual hours/week&       21.02&       20.79&       21.67&       21.01&        0.65&        0.45\\
Usual weekly earn.&      104.03&      117.69&      109.92&      343.24&        5.90&        5.01\\


==> empiric_tbls_figs/sum_stats/old/sumstats_unweighted_5.tex <==
 
Week 52 hours&       17.95&       23.65&       15.27&       22.56&       -2.68&        0.50\\
Week 104 hours&       22.25&       26.29&       22.57&       26.14&        0.32&        0.56\\
Week 156 hours&       24.20&       26.37&       25.84&       26.45&        1.64&        0.57\\
Week 208 hours&       26.39&       26.58&       27.71&       25.61&        1.32&        0.56\\
Week 52 earn.&      105.96&      164.23&       91.55&      149.13&      -14.41&        3.39\\
Week 104 earn.&      153.03&      208.69&      156.76&      199.05&        3.73&        4.39\\
Week 156 earn.&      184.63&      228.29&      203.69&      239.45&       19.06&        4.98\\
Week 208 earn.&      206.53&      235.41&      227.52&      249.33&       20.99&        5.16\\


==> empiric_tbls_figs/sum_stats/old/sumstats_unweighted_6.tex <==
 
Total 4 yr. earn.&    30659.18&    27365.85&    30773.50&    26403.90&      114.32&      577.74\\


==> empiric_tbls_figs/sum_stats/old/sumstats_unweighted_7.tex <==
 
Sample size &        3599&           &        5546&           &        9145&           \\


==> empiric_tbls_figs/types_dist/old/dist_wk135.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{cc}}
\toprule
            &     Control&     Treated&  Difference&ln(Hourly wage)\\
\midrule
H=1, R=1, V=1&        0.36&        0.38&        0.02&        2.05\\
            &    \{0.48\}&    \{0.49\}&      (0.02)&    \{0.34\}\\
            &            &            &      [0.30]&            \\
H=1, R=1, V=0&        0.03&        0.03&       -0.00&        2.06\\
            &    \{0.16\}&    \{0.16\}&      (0.01)&    \{0.34\}\\
            &            &            &      [0.92]&            \\
H=1, R=0, V=1&        0.11&        0.10&       -0.01&        1.98\\
            &    \{0.31\}&    \{0.30\}&      (0.01)&    \{0.32\}\\
            &            &            &      [0.62]&            \\
H=1, R=0, V=0&        0.04&        0.04&        0.01&        1.88\\
            &    \{0.19\}&    \{0.21\}&      (0.01)&    \{0.41\}\\
            &            &            &      [0.26]&            \\
H=0, R=1, V=1&        0.03&        0.03&       -0.00&        1.91\\
            &    \{0.17\}&    \{0.16\}&      (0.01)&    \{0.29\}\\
            &            &            &      [0.67]&            \\
H=0, R=1, V=0&        0.02&        0.02&       -0.00&        1.89\\
            &    \{0.15\}&    \{0.14\}&      (0.01)&    \{0.33\}\\
            &            &            &      [0.40]&            \\
H=0, R=0, V=1&        0.08&        0.06&       -0.02&        1.85\\
            &    \{0.27\}&    \{0.24\}&      (0.01)&    \{0.32\}\\
            &            &            &      [0.05]&            \\
H=0, R=0, V=0&        0.33&        0.34&        0.00&        1.86\\
            &    \{0.47\}&    \{0.47\}&      (0.02)&    \{0.36\}\\
            &            &            &      [0.80]&            \\
\midrule
Sample Size &        2454&        3778&        6232&            \\
\bottomrule
\multicolumn{5}{l}{\footnotesize Note: Standard deviations in \{ \}, standard errors in ( ), p-values in  [ ].}\\
\multicolumn{5}{l}{\footnotesize ln(Hourly Wage) presents the pooled mean by type; hourly wage is}\\
\multicolumn{5}{l}{\footnotesize calculated as weekly earnings divided by weekly hours for the employed.}\\
\end{tabular}
\caption{Distribution of job types at week 135 (conditional on employment) \label{typedist135}}
\end{table}


==> empiric_tbls_figs/types_dist/old/dist_wk180.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{cc}}
\toprule
            &     Control&     Treated&  Difference&ln(Hourly wage)\\
\midrule
H=1, R=1, V=1&        0.37&        0.39&        0.02&        2.12\\
            &    \{0.48\}&    \{0.49\}&      (0.02)&    \{0.34\}\\
            &            &            &      [0.24]&            \\
H=1, R=1, V=0&        0.02&        0.03&        0.01&        2.12\\
            &    \{0.14\}&    \{0.18\}&      (0.01)&    \{0.32\}\\
            &            &            &      [0.07]&            \\
H=1, R=0, V=1&        0.12&        0.10&       -0.01&        2.02\\
            &    \{0.32\}&    \{0.31\}&      (0.01)&    \{0.31\}\\
            &            &            &      [0.25]&            \\
H=1, R=0, V=0&        0.04&        0.04&       -0.00&        1.91\\
            &    \{0.19\}&    \{0.19\}&      (0.01)&    \{0.46\}\\
            &            &            &      [0.94]&            \\
H=0, R=1, V=1&        0.03&        0.03&        0.00&        2.00\\
            &    \{0.17\}&    \{0.17\}&      (0.01)&    \{0.36\}\\
            &            &            &      [0.82]&            \\
H=0, R=1, V=0&        0.01&        0.02&        0.01&        1.93\\
            &    \{0.11\}&    \{0.14\}&      (0.00)&    \{0.37\}\\
            &            &            &      [0.19]&            \\
H=0, R=0, V=1&        0.09&        0.07&       -0.01&        1.90\\
            &    \{0.28\}&    \{0.26\}&      (0.01)&    \{0.33\}\\
            &            &            &      [0.15]&            \\
H=0, R=0, V=0&        0.33&        0.32&       -0.01&        1.87\\
            &    \{0.47\}&    \{0.46\}&      (0.02)&    \{0.40\}\\
            &            &            &      [0.51]&            \\
\midrule
Sample Size &        2454&        3778&        6232&            \\
\bottomrule
\multicolumn{5}{l}{\footnotesize Note: Standard deviations in \{ \}, standard errors in ( ), p-values in  [ ].}\\
\multicolumn{5}{l}{\footnotesize ln(Hourly Wage) presents the pooled mean by type; hourly wage is}\\
\multicolumn{5}{l}{\footnotesize calculated as weekly earnings divided by weekly hours for the employed.}\\
\end{tabular}
\caption{Distribution of job types at week 180 (conditional on employment) \label{typedist180}}
\end{table}


==> empiric_tbls_figs/types_dist/old/dist_wk208.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{cc}}
\toprule
            &     Control&     Treated&  Difference&ln(Hourly wage)\\
\midrule
H=1, R=1, V=1&        0.37&        0.41&        0.04&        2.13\\
            &    \{0.48\}&    \{0.49\}&      (0.02)&    \{0.32\}\\
            &            &            &      [0.02]&            \\
H=1, R=1, V=0&        0.03&        0.03&        0.00&        2.08\\
            &    \{0.16\}&    \{0.17\}&      (0.01)&    \{0.33\}\\
            &            &            &      [0.64]&            \\
H=1, R=0, V=1&        0.12&        0.11&       -0.01&        2.01\\
            &    \{0.32\}&    \{0.31\}&      (0.01)&    \{0.34\}\\
            &            &            &      [0.36]&            \\
H=1, R=0, V=0&        0.04&        0.04&       -0.00&        1.94\\
            &    \{0.20\}&    \{0.19\}&      (0.01)&    \{0.45\}\\
            &            &            &      [0.57]&            \\
H=0, R=1, V=1&        0.03&        0.03&       -0.00&        2.00\\
            &    \{0.17\}&    \{0.16\}&      (0.01)&    \{0.38\}\\
            &            &            &      [0.79]&            \\
H=0, R=1, V=0&        0.01&        0.02&        0.00&        1.93\\
            &    \{0.12\}&    \{0.13\}&      (0.00)&    \{0.33\}\\
            &            &            &      [0.51]&            \\
H=0, R=0, V=1&        0.09&        0.07&       -0.02&        1.92\\
            &    \{0.28\}&    \{0.26\}&      (0.01)&    \{0.27\}\\
            &            &            &      [0.11]&            \\
H=0, R=0, V=0&        0.31&        0.30&       -0.02&        1.88\\
            &    \{0.46\}&    \{0.46\}&      (0.02)&    \{0.43\}\\
            &            &            &      [0.35]&            \\
\midrule
Sample Size &        2454&        3778&        6232&            \\
\bottomrule
\multicolumn{5}{l}{\footnotesize Note: Standard deviations in \{ \}, standard errors in ( ), p-values in  [ ].}\\
\multicolumn{5}{l}{\footnotesize ln(Hourly Wage) presents the pooled mean by type; hourly wage is}\\
\multicolumn{5}{l}{\footnotesize calculated as weekly earnings divided by weekly hours for the employed.}\\
\end{tabular}
\caption{Distribution of job types at week 208 (conditional on employment) \label{typedist208}}
\end{table}


==> empiric_tbls_figs/types_dist/old/dist_wk45.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{cc}}
\toprule
            &     Control&     Treated&  Difference&ln(Hourly wage)\\
\midrule
H=1, R=1, V=1&        0.21&        0.26&        0.04&        1.84\\
            &    \{0.41\}&    \{0.44\}&      (0.02)&    \{0.33\}\\
            &            &            &      [0.03]&            \\
H=1, R=1, V=0&        0.03&        0.02&       -0.01&        1.77\\
            &    \{0.18\}&    \{0.15\}&      (0.01)&    \{0.34\}\\
            &            &            &      [0.15]&            \\
H=1, R=0, V=1&        0.08&        0.11&        0.02&        1.81\\
            &    \{0.28\}&    \{0.31\}&      (0.01)&    \{0.22\}\\
            &            &            &      [0.10]&            \\
H=1, R=0, V=0&        0.06&        0.04&       -0.02&        1.68\\
            &    \{0.24\}&    \{0.19\}&      (0.01)&    \{0.29\}\\
            &            &            &      [0.02]&            \\
H=0, R=1, V=1&        0.03&        0.02&       -0.00&        1.69\\
            &    \{0.16\}&    \{0.15\}&      (0.01)&    \{0.22\}\\
            &            &            &      [0.81]&            \\
H=0, R=1, V=0&        0.03&        0.03&       -0.00&        1.70\\
            &    \{0.17\}&    \{0.16\}&      (0.01)&    \{0.31\}\\
            &            &            &      [0.67]&            \\
H=0, R=0, V=1&        0.08&        0.07&       -0.01&        1.65\\
            &    \{0.27\}&    \{0.25\}&      (0.01)&    \{0.26\}\\
            &            &            &      [0.34]&            \\
H=0, R=0, V=0&        0.47&        0.46&       -0.02&        1.66\\
            &    \{0.50\}&    \{0.50\}&      (0.02)&    \{0.34\}\\
            &            &            &      [0.51]&            \\
\midrule
Sample Size &        2454&        3778&        6232&            \\
\bottomrule
\multicolumn{5}{l}{\footnotesize Note: Standard deviations in \{ \}, standard errors in ( ), p-values in  [ ]}\\
\end{tabular}
\caption{Distribution of job types at week 45 (conditional on employment) \label{typedist45}}
\end{table}


==> empiric_tbls_figs/types_dist/old/dist_wk90.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{cc}}
\toprule
            &     Control&     Treated&  Difference&ln(Hourly wage)\\
\midrule
H=1, R=1, V=1&        0.29&        0.33&        0.04&        1.98\\
            &    \{0.45\}&    \{0.47\}&      (0.02)&    \{0.32\}\\
            &            &            &      [0.03]&            \\
H=1, R=1, V=0&        0.03&        0.02&       -0.01&        1.95\\
            &    \{0.17\}&    \{0.14\}&      (0.01)&    \{0.31\}\\
            &            &            &      [0.13]&            \\
H=1, R=0, V=1&        0.11&        0.11&       -0.00&        1.90\\
            &    \{0.31\}&    \{0.31\}&      (0.01)&    \{0.25\}\\
            &            &            &      [0.88]&            \\
H=1, R=0, V=0&        0.05&        0.05&       -0.00&        1.83\\
            &    \{0.22\}&    \{0.21\}&      (0.01)&    \{0.28\}\\
            &            &            &      [0.76]&            \\
H=0, R=1, V=1&        0.03&        0.03&        0.00&        1.89\\
            &    \{0.17\}&    \{0.18\}&      (0.01)&    \{0.30\}\\
            &            &            &      [0.59]&            \\
H=0, R=1, V=0&        0.02&        0.01&       -0.01&        1.82\\
            &    \{0.14\}&    \{0.12\}&      (0.01)&    \{0.24\}\\
            &            &            &      [0.32]&            \\
H=0, R=0, V=1&        0.07&        0.09&        0.02&        1.76\\
            &    \{0.26\}&    \{0.29\}&      (0.01)&    \{0.31\}\\
            &            &            &      [0.13]&            \\
H=0, R=0, V=0&        0.40&        0.36&       -0.04&        1.76\\
            &    \{0.49\}&    \{0.48\}&      (0.02)&    \{0.31\}\\
            &            &            &      [0.03]&            \\
\midrule
Sample Size &        2454&        3778&        6232&            \\
\bottomrule
\multicolumn{5}{l}{\footnotesize Note: Standard deviations in \{ \}, standard errors in ( ), p-values in  [ ].}\\
\multicolumn{5}{l}{\footnotesize ln(Hourly Wage) presents the pooled mean by type; hourly wage is}\\
\multicolumn{5}{l}{\footnotesize calculated as weekly earnings divided by weekly hours for the employed.}\\
\end{tabular}
\caption{Distribution of job types at week 90 (conditional on employment) \label{typedist90}}
\end{table}


==> empiric_tbls_figs/types_dist/old/typesdist_wk135_unweighted_A.tex <==
            &        Mean&          S.D.&        Mean&          S.D.&  Difference&          S.E.&ln(Hourly wage)&          S.D.\\
\midrule
H=1, R=1, V=1&      0.3617&      0.4807&      0.3818&      0.4860&      0.0201&      0.0192&      2.0480&      0.3379\\
H=1, R=1, V=0&      0.0268&      0.1615&      0.0261&      0.1596&     -0.0006&      0.0064&      2.0623&      0.3402\\
H=1, R=0, V=1&      0.1070&      0.3093&      0.1010&      0.3014&     -0.0061&      0.0122&      1.9843&      0.3233\\
H=1, R=0, V=0&      0.0357&      0.1856&      0.0445&      0.2063&      0.0089&      0.0077&      1.8826&      0.4126\\
H=0, R=1, V=1&      0.0307&      0.1727&      0.0279&      0.1648&     -0.0028&      0.0068&      1.9122&      0.2927\\
H=0, R=1, V=0&      0.0238&      0.1525&      0.0190&      0.1366&     -0.0048&      0.0058&      1.8929&      0.3297\\
H=0, R=0, V=1&      0.0813&      0.2734&      0.0618&      0.2408&     -0.0195&      0.0104&      1.8533&      0.3210\\
H=0, R=0, V=0&      0.3330&      0.4715&      0.3379&      0.4731&      0.0049&      0.0188&      1.8603&      0.3637\\


==> empiric_tbls_figs/types_dist/old/typesdist_wk135_unweighted_B.tex <==
 
Sample size &        2454&           &        3778&           &           &           &        6232&           \\


==> empiric_tbls_figs/types_dist/old/typesdist_wk180_unweighted_A.tex <==
            &        Mean&          S.D.&        Mean&          S.D.&  Difference&          S.E.&ln(Hourly wage)&          S.D.\\
\midrule
H=1, R=1, V=1&      0.3671&      0.4822&      0.3880&      0.4874&      0.0210&      0.0177&      2.1197&      0.3418\\
H=1, R=1, V=0&      0.0209&      0.1431&      0.0317&      0.1753&      0.0108&      0.0057&      2.1241&      0.3163\\
H=1, R=0, V=1&      0.1179&      0.3226&      0.1047&      0.3062&     -0.0132&      0.0116&      2.0230&      0.3090\\
H=1, R=0, V=0&      0.0393&      0.1944&      0.0388&      0.1931&     -0.0005&      0.0071&      1.9106&      0.4638\\
H=0, R=1, V=1&      0.0293&      0.1686&      0.0307&      0.1725&      0.0014&      0.0062&      1.9962&      0.3572\\
H=0, R=1, V=0&      0.0125&      0.1113&      0.0186&      0.1352&      0.0061&      0.0044&      1.9347&      0.3658\\
H=0, R=0, V=1&      0.0861&      0.2807&      0.0720&      0.2585&     -0.0142&      0.0100&      1.8978&      0.3305\\
H=0, R=0, V=0&      0.3269&      0.4693&      0.3156&      0.4649&     -0.0114&      0.0171&      1.8660&      0.4046\\


==> empiric_tbls_figs/types_dist/old/typesdist_wk180_unweighted_B.tex <==
 
Sample size &        2454&           &        3778&           &           &           &        6232&           \\


==> empiric_tbls_figs/types_dist/old/typesdist_wk208_unweighted_A.tex <==
            &        Mean&          S.D.&        Mean&          S.D.&  Difference&          S.E.&ln(Hourly wage)&          S.D.\\
\midrule
H=1, R=1, V=1&      0.3689&      0.4827&      0.4092&      0.4918&      0.0403&      0.0172&      2.1283&      0.3249\\
H=1, R=1, V=0&      0.0265&      0.1606&      0.0292&      0.1683&      0.0027&      0.0058&      2.0793&      0.3269\\
H=1, R=0, V=1&      0.1183&      0.3231&      0.1082&      0.3107&     -0.0101&      0.0113&      2.0110&      0.3406\\
H=1, R=0, V=0&      0.0420&      0.2007&      0.0381&      0.1915&     -0.0039&      0.0070&      1.9413&      0.4495\\
H=0, R=1, V=1&      0.0288&      0.1673&      0.0273&      0.1629&     -0.0015&      0.0059&      2.0016&      0.3770\\
H=0, R=1, V=0&      0.0140&      0.1176&      0.0169&      0.1291&      0.0029&      0.0043&      1.9250&      0.3256\\
H=0, R=0, V=1&      0.0872&      0.2822&      0.0720&      0.2585&     -0.0152&      0.0097&      1.9246&      0.2717\\
H=0, R=0, V=0&      0.3144&      0.4645&      0.2992&      0.4580&     -0.0152&      0.0163&      1.8814&      0.4318\\


==> empiric_tbls_figs/types_dist/old/typesdist_wk208_unweighted_B.tex <==
 
Sample size &        2454&           &        3778&           &           &           &        6232&           \\


==> empiric_tbls_figs/types_dist/old/typesdist_wk90_unweighted_A.tex <==
            &        Mean&          S.D.&        Mean&          S.D.&  Difference&          S.E.&ln(Hourly wage)&          S.D.\\
\midrule
H=1, R=1, V=1&      0.2891&      0.4536&      0.3314&      0.4709&      0.0423&      0.0198&      1.9849&      0.3186\\
H=1, R=1, V=0&      0.0304&      0.1717&      0.0203&      0.1409&     -0.0101&      0.0069&      1.9502&      0.3134\\
H=1, R=0, V=1&      0.1091&      0.3120&      0.1071&      0.3093&     -0.0020&      0.0134&      1.9038&      0.2526\\
H=1, R=0, V=0&      0.0506&      0.2193&      0.0478&      0.2133&     -0.0029&      0.0093&      1.8266&      0.2835\\
H=0, R=1, V=1&      0.0292&      0.1686&      0.0333&      0.1794&      0.0040&      0.0074&      1.8871&      0.2970\\
H=0, R=1, V=0&      0.0191&      0.1370&      0.0137&      0.1165&     -0.0054&      0.0056&      1.8209&      0.2371\\
H=0, R=0, V=1&      0.0731&      0.2605&      0.0912&      0.2880&      0.0181&      0.0117&      1.7574&      0.3104\\
H=0, R=0, V=0&      0.3993&      0.4900&      0.3553&      0.4788&     -0.0440&      0.0209&      1.7619&      0.3071\\


==> empiric_tbls_figs/types_dist/old/typesdist_wk90_unweighted_B.tex <==
 
Sample size &        2454&           &        3778&           &           &           &        6232&           \\


==> empiric_tbls_figs/workadv_bounds/sumstats_ohio_2.tex <==
 
Target sector share&        0.47&        0.50&        0.51&        0.50&        0.03&        0.05\\


==> empiric_tbls_figs/workadv_bounds/sumstats_okla_2.tex <==
 
Target sector share&        0.31&        0.46&        0.44&        0.50&        0.14&        0.04\\

